How Contaminated Is Your Benchmark? Quantifying Dataset Leakage in Large Language Models with Kernel Divergence

Dataset contamination, where evaluation datasets overlap with pre-training corpora, inflates performance metrics and undermines the reliability of model evaluations. Measuring dataset contamination thus becomes essential to ensure that performance evaluations genuinely reflect a model's ability to generalize to unseen data, rather than relying on memorized examples. To address this problem, we propose Kernel Divergence Score (KDS), a novel method that evaluates dataset contamination by computing the divergence between the kernel similarity matrix of sample embeddings, before and after fine-tuning on the benchmark dataset. Leveraging the insight that fine-tuning affects unseen samples more significantly than seen ones, KDS provides a reliable measure of contamination. Through extensive experiments on controlled contamination scenarios, KDS demonstrates a near-perfect correlation with contamination levels and outperforms existing baselines. Additionally, we perform comprehensive ablation studies to analyze the impact of key design choices, providing deeper insights into the components and effectiveness of KDS. These ablations highlight the importance of leveraging fine-grained kernel-based information and confirm the reliability of the proposed framework across diverse datasets and settings. Code is released in https://github.com/deeplearning-wisc/kernel-divergence-score.

==> 5_Analysis/definition.tex <==

\noindent\textbf{Definition 3.} \textit{(\textbf{Fine-tuned Score Deviation}) is the difference of scores before and after supervised fine-tuning, averaged across samples:}
\begin{equation}
    \frac{1}{n}\sum_{i=1}^n S(\mathbf{x}_i; \theta) - S(\mathbf{x}_i; \theta'),
\end{equation}
\textit{where $\mathbf{x}_i$ is the $i$-th sample in the dataset, $S(\cdot;\cdot)$ is an existing scoring function~(e.g., Min-K\% or Perplexity Score), and $\theta, \theta'$ are models before and after fine-tuning, respectively.}~\cite{zhang2024fine}


\input{B_Figures/req2}
In comparison to the detector-based scoring methods, we evaluate our Kernel Divergence Score, in addition to alternative scoring approaches that alsp leverage the fine-grained information of kernels.
In all their definitions below, let $Z, Z' \in \mathbb{R}^{n \times d}$ be the embeddings before and after supervised fine-tuning, respectively, where $Z_i, Z_i' \in \mathbb{R}^{1 \times d}$ are row vectors.

\noindent\textbf{Definition 5.} \textit{(\textbf{KDE KL Divergence}) is the Kullback-Leibler divergence of the Kernel Density Estimator~(KDE):}
\begin{equation}
    \text{KLD}\bigg(\frac{1}{E}\sum_{i=1}^n\Phi(Z)_{i,j} \; \bigg\vert \; \frac{1}{E'}\sum_{i=1}^n\Phi(Z')_{i,j}\bigg),
\end{equation}
\textit{where $\Phi(\cdot)$ is the RBF kernel, $Z, Z'$ are normalized model embeddings, $E = \sum_{i,j} \Phi(Z)_{i,j}$ and $E' = \sum_{i,j} \Phi(Z')_{i,j}$.}

\noindent\textbf{Definition 6.} \textit{(\textbf{Maximum Mean Discrepancy$^2$}) is the squared value of the maximum mean discrepancy~(MMD):}
\begin{equation}
    \text{MMD}(Z, Z') = \sup_{f \in \mathcal{H}}\bigg(\mathbb{E}_{Z}[f(Z)] - \mathbb{E}_{Z'}[f(Z')]\bigg),
\end{equation}
\textit{where $\mathcal{H}$ is the reproducing kernel Hilbert space~(RKHS). In practice, }
\begin{equation}
    \mathbb{E}_Z[k(Z_i, Z_i)] + \mathbb{E}_{Z'}[k(Z_i', Z_i')] - 2 \mathbb{E}_{Z,Z'}[k(Z_i, Z_i')]
\end{equation}
\textit{is computed as the MMD$^2$, where $k$ is the kernel function.}~\cite{gretton2012kernel}


\noindent\textbf{Definition 7.} \textit{(\textbf{Centered Kernel Alignment}) is defined as}
\begin{equation}
    1 - \frac{||Z^\top Z'||_\text{F}^2}{||Z^\top Z||_\text{F} ||Z'^\top Z'||_\text{F}},
\end{equation}
\textit{where $Z, Z'$ are zero-centered embeddings.}~\cite{kornblith2019similarity}



\noindent\textbf{Definition 8.} \textit{(\textbf{Dot-product Kernel MSE}) is the mean squared error of paired dot-product kernels:}
\begin{equation}
    \frac{1}{n^2}||Z Z^\top - Z' Z'^\top||_\text{F}^2,
\end{equation}
\textit{where $n$ is the number of samples.}

\noindent\textbf{Definition 9.} \textit{(\textbf{Cosine Similarity Kernel MSE}) is the mean squared error of paired cosine similarity kernels.}
\begin{equation}
    \frac{1}{n^2}\bigg\Vert\frac{Z Z^\top}{||Z||_2^2} - \frac{Z' Z'^\top}{||Z'||_2^2}\bigg\Vert_\text{F}^2,
\end{equation}
\textit{where $n$ is the number of samples.}


\noindent\textbf{Definition 10.} \textit{(\textbf{RBF Kernel MSE}) is the mean squared error of paired radial basis function~(RBF) kernels.}
\begin{equation}
    \frac{1}{n^2}||\Phi(Z) - \Phi(Z')||_\text{F}^2,
\end{equation}
\textit{where $n$ is the number of samples, $\Phi$ is the RBF kernel, and $Z, Z'$ are normalized model embeddings.}

We subtract the original Centered Kernel Alignment~(CKA) value from 1 to ensure that the measure's trend aligns with the contamination rate trends observed in other kernel-based baselines.
Note that this does not affect the general property of the measure.
Further implementation details and hyperparameters for each baseline are provided in Appendix~\ref{}.


==> B_Figures/prelim.tex <==

\begin{figure}[t!]
    \begin{center}
    \includegraphics[width=\linewidth]{B_Figures/figs/prelim2.png}
    \end{center}
    \vspace{-3mm}
    \caption{\textbf{Existing scoring functions lack monotonicity under increasing contamination levels.} The experiments are conducted on WikiMIA~\cite{shidetecting} with Mistral-7B-Instruct-v0.2~\cite{jiang2023mistral}. The $x$-axis is the ground-truth contamination rate of the test set, and the $y$-axis shows the normalized scores of each method. The results illustrate that existing scores do not exhibit a monotonic trend w.r.t. the contamination rate.}
\label{fig:prelim}
\end{figure}

==> B_Figures/req2.tex <==

\begin{figure*}[t!]
    \begin{center}
    \includegraphics[width=\linewidth]{B_Figures/figs/req2_2.png}
    \end{center}
    \vspace{-5mm}
    \caption{\textbf{Consistency Requirement Compliance Evaluation.} Light bars are detector-based baselines, and darker bars are kernel-based. The darkest bar is our Kernel Divergence Score. (a) To evaluate how different datasets sampled from the same distribution affect score magnitudes, we present the average MAPE of baseline scores measured across five independent runs. (b) To assess the effect of dataset size on score magnitudes, we compute the average MAPE between WikiMIA subsets of size 700 and 350.}
\label{fig:req2}
\end{figure*}


==> B_Figures/trend_full.tex <==

\begin{figure}[h]
    \begin{center}
    \includegraphics[width=\linewidth]{B_Figures/figs/trend_full.pdf}
    \end{center}
    \vspace{-3mm}
    \caption{\textbf{More trends of Kernel Divergence Scores on WikiMIA.}}
\label{fig:trend}
\end{figure}
